Neural Elevation Models for Terrain Mapping and Path Planning

This work introduces Neural Elevations Models (NEMos), which adapt Neural Radiance Fields to a 2.5D continuous and differentiable terrain model. In contrast to traditional terrain representations such as digital elevation models, NEMos can be readily generated from imagery, a low-cost data source, and provide a lightweight representation of terrain through an implicit continuous and differentiable height field. We propose a novel method for jointly training a height field and radiance field within a NeRF framework, leveraging quantile regression. Additionally, we introduce a path planning algorithm that performs gradient-based optimization of a continuous cost function for minimizing distance, slope changes, and control effort, enabled by differentiability of the height field. We perform experiments on simulated and real-world terrain imagery, demonstrating NEMos ability to generate high-quality reconstructions and produce smoother paths compared to discrete path planning methods. Future work will explore the incorporation of features and semantics into the height field, creating a generalized terrain model.

==> sections/outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]
    \1 Abstract (0.25 pg)
    \1 Introduction (0.5 pg)
        \2 
    \1 Related work (0.75 pg)
        \2 
            
    \1 Problem statement (<0.25 pg)
        \2 
    \1 Approach (2 pg)
        \2 
            
    \1 Results (2 pg)
        \2
    
        
\end{outline}

==> sections/related_work.tex <==
\section{Related Work}


% DEMs
% - Grid (most common)
% - Mesh (Triangulated Irregular Network or TIN)
% - DSM (Digital Surface Model) - capture vegetation and buildings
% - DTM (Digital Terrain Model) - bare-earth DEM
% - Digitized contour maps

% Terrain modeling/path planning
% - Fitting continuous functions (polynomials, trig, exp, radial basis, bezier surfaces, etc.) to model terrain
\cite{carsten2007global} - Mars global path planning, Field D*

% NeRFs
% - Sat NeRF
% - Bungee NeRF
Sat-NeRF \cite{mari2022sat}, BungeeNeRF \cite{xiangli2022bungeenerf}
 - Methods for large scale NeRFs, but don't propose a 2.5D representation


% NeRF path planning
% - Nerf-Nav
% - ION Rover nerf
\cite{adamkiewicz2022vision} 
\cite{dai2023neural}














